Classifier Pool Generation based on a Two-level Diversity Approach

This paper describes a classifier pool generation method guided by the diversity estimated on the data complexity and classifier decisions. First, the behavior of complexity measures is assessed by considering several subsamples of the dataset. The complexity measures with high variability across the subsamples are selected for posterior pool adaptation, where an evolutionary algorithm optimizes diversity in both complexity and decision spaces. A robust experimental protocol with 28 datasets and 20 replications is used to evaluate the proposed method. Results show significant accuracy improvements in 69.4% of the experiments when Dynamic Classifier Selection and Dynamic Ensemble Selection methods are applied.

==> result_table_disp.tex <==
\begin{table*}[!t]
\caption{Comparison of the proposed method for pool generation based on diversity in the complexity space. The results of the mean and standard deviation winners are highlighted.The asterisk represents where there was difference in Wilcoxon}
\label{tab:tabresult}
\resizebox{\textwidth}{!}{
\scalefont{0.6}
\centering
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{ c c c c c c c c c c c c c c c}

\hline
\textbf{} & \multicolumn{ 2}{c}{\textbf{ALL}} & \multicolumn{ 2}{c}{\textbf{Knora-U}} & \multicolumn{ 2}{c}{\textbf{Knora-E}} & \multicolumn{ 2}{c}{\textbf{OLA}} & \multicolumn{ 2}{c}{\textbf{LCA}} & \multicolumn{ 2}{c}{\textbf{RANK}} & \multicolumn{ 2}{c}{\textbf{META}} \\ 
\hline
\textbf{Data} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} & \textbf{Bagging} & \textbf{PGCS} \\
\hline
    % 06 & Faults & 1941 &  27  & 7       & UCI     \\
\textbf{1} & \textbf{86.9 (2.2)} & 86.8 (1.9) & 86.8 (2.3) & \textbf{86.9 (1.9)} & 83.1 (3.4) & \textbf{84.5 (3.4)} & 83.8 (2.6) & \textbf{84.6 (2.3)} & 83.5 (2.2) & \textbf{84.5 (2.4)} & 81.9 (3.6) & \textbf{83.7 (2.7)} & 85.8 (2.4) & \textbf{86.2 (2.0)} \\ 
\textbf{2} & \textbf{84.4 (1.3)} & \textbf{84.4 (1.6)} & \textbf{96.2 (1.0)*} & 94.3 (1.6) & \textbf{97.0 (0.8)*} & 96.5 (1.3) & \textbf{97.4 (0.6)*} & 96.7 (1.1) & \textbf{95.7 (1.0)} & 95.5 (1.0) & \textbf{96.8 (0.7)*} & 96.3 (1.3) & \textbf{93.1 (1.5)*} & 92.0 (2.2) \\ 
\textbf{3} & \textbf{77.8 (2.0)*} & 74.1 (4.5) & \textbf{78.8 (1.9)} & 77.6 (3.4) & \textbf{70.2 (3.5)} & 69.9 (3.4) & 74.9 (3.8) & \textbf{75.3 (2.5)} & \textbf{71.8 (6.3)} & 71.3 (5.6) & \textbf{69.9 (3.7)} & \textbf{69.9 (3.3)} & 76.1 (1.1) & \textbf{76.2 (1.0)} \\ 
\textbf{4} & \textbf{81.2 (24.3)} & 80.9 (24.2) & \textbf{89.0 (2.1)} & 88.8 (2.1) & \textbf{89.6 (1.5)} & 89.4 (1.5) & \textbf{89.3 (1.3)} & 89.0 (1.5) & 86.4 (1.7) & \textbf{86.9 (1.9)} & \textbf{89.1 (1.3)} & 88.9 (1.5) & 89.0 (1.1) & \textbf{89.1 (1.5)} \\ 
\textbf{5} & \textbf{76.4 (2.8)} & 76.0 (3.5) & \textbf{76.8 (2.7)} & 75.9 (3.2) & \textbf{72.5 (2.8)*} & 72.0 (2.3) & 72.7 (3.1) & \textbf{73.2 (2.6)} & 68.5 (3.8) & \textbf{71.0 (4.6)*} & \textbf{72.1 (3.3)} & 71.6 (2.3) & 74.4 (2.3) & \textbf{74.8 (2.4)} \\ 
\textbf{6} & \textbf{69.3 (1.3)*} & 68.5 (1.6) & \textbf{71.5 (1.4)} & 70.1 (1.5) & \textbf{69.2 (1.8)*} & 68.9 (1.7) & 67.3 (1.4) & \textbf{68.2 (2.0)*} & 62.0 (2.0) & \textbf{63.5 (2.0)*} & \textbf{67.7 (2.0)} & 67.3 (2.1) & \textbf{70.6 (1.3)*} & 69.8 (1.9) \\ 
\textbf{7} & \textbf{76.2 (2.3)} & 75.3 (2.9) & \textbf{76.3 (2.2)} & 75.4 (2.6) & 71.8 (2.2) & \textbf{71.9 (2.2)} & 70.9 (2.3) & \textbf{71.9 (2.6)} & 68.1 (2.7) & \textbf{70.4 (1.9)*} & 70.2 (2.2) & \textbf{70.6 (2.7)} & 72.6 (1.5) & \textbf{74.4 (2.0)*} \\ 
\textbf{8} & 74.5 (2.7) & \textbf{75.7 (3.1)*} & 74.9 (2.2) & \textbf{75.7 (2.3)} & 66.1 (5.4) & \textbf{67.0 (5.6)*} & 69.9 (5.4) & \textbf{70.7 (5.4)} & 70.9 (5.9) & \textbf{72.0 (6.0)} & 64.7 (5.7) & \textbf{66.6 (5.5)} & \textbf{73.6 (1.2)} & \textbf{73.6 (1.4)} \\ 
\textbf{9} & \textbf{83.0 (3.1)} & 82.2 (3.8) & \textbf{83.3 (2.8)} & 82.3 (3.8) & 78.4 (3.6) & \textbf{79.0 (4.3)} & 76.9 (4.0) & \textbf{78.4 (5.1)} & 76.0 (4.5) & \textbf{79.4 (4.2)*} & 75.8 (4.0) & \textbf{77.9 (5.1)} & \textbf{83.6 (3.5)} & 82.5 (3.7) \\ 
\textbf{10} & 70.5 (2.8) & \textbf{70.6 (1.8)} & \textbf{71.1 (2.4)} & \textbf{71.1 (2.0)} & \textbf{69.5 (3.3)} & 68.9 (3.8) & \textbf{69.3 (2.1)} & 69.1 (3.4) & 67.8 (4.0) & \textbf{69.0 (3.1)} & \textbf{68.4 (3.0)} & 68.0 (3.4) & \textbf{70.9 (2.3)} & 70.1 (2.7) \\ 
\textbf{11} & 82.8 (3.9) & \textbf{83.6 (4.2)} & \textbf{83.3 (3.8)} & 83.1 (3.7) & \textbf{80.8 (3.8)} & 79.5 (3.9) & \textbf{81.4 (5.8)} & \textbf{81.4 (4.9)} & \textbf{78.9 (5.4)} & 78.2 (5.2) & 79.4 (5.5) & \textbf{79.9 (4.2)} & \textbf{83.4 (5.4)} & 82.5 (4.4) \\ 
\textbf{12} & 72.6 (2.2) & \textbf{73.9 (2.5)*} & 73.5 (2.6) & \textbf{73.8 (2.8)*} & 64.5 (4.3) & \textbf{67.5 (4.9)} & 66.0 (4.5) & \textbf{69.3 (4.9)*} & 67.5 (5.1) & \textbf{72.3 (3.5)*} & 62.8 (4.5) & \textbf{66.3 (5.8)*} & 70.5 (3.1) & \textbf{71.2 (3.7)} \\ 
\textbf{13} & \textbf{82.7 (1.9)} & 82.3 (1.4) & \textbf{95.1 (1.0)} & 93.6 (1.4) & \textbf{96.0 (0.8)*} & 95.7 (0.9) & \textbf{96.6 (0.5)} & 96.3 (0.9) & \textbf{93.0 (1.2)} & \textbf{93.0 (1.0)} & \textbf{96.0 (0.7)*} & 95.5 (0.9) & \textbf{94.3 (1.0)*} & 93.3 (1.5) \\ 
\textbf{14} & \textbf{68.6 (3.9)} & 66.0 (5.4) & \textbf{69.9 (3.4)} & 67.4 (4.7) & \textbf{65.8 (3.5)*} & 64.5 (4.6) & 65.0 (5.4) & \textbf{67.4 (4.7)*} & 55.3 (3.4) & \textbf{55.6 (5.8)} & \textbf{64.4 (4.2)} & 63.8 (5.2) & \textbf{67.0 (5.3)} & 65.6 (3.5) \\ 
\textbf{15} & \textbf{83.0 (2.2)} & 82.5 (2.0) & \textbf{83.0 (2.0)} & 82.8 (2.0) & 77.2 (2.9) & \textbf{77.7 (2.2)} & 81.3 (2.4) & \textbf{81.4 (2.8)} & 78.2 (4.7) & \textbf{79.8 (5.1)} & 77.4 (2.7) & \textbf{77.5 (2.3)} & 79.5 (3.1) & \textbf{80.8 (3.2)*} \\ 
\textbf{16} & 79.3 (3.5) & \textbf{82.7 (3.3)*} & 81.8 (3.0) & \textbf{83.8 (3.4)*} & 88.6 (2.7) & \textbf{90.2 (3.3)*} & 86.6 (3.6) & \textbf{88.1 (4.1)} & 73.1 (4.4) & \textbf{76.7 (4.5)*} & 86.1 (3.7) & \textbf{87.4 (3.4)} & 91.2 (4.9) & \textbf{92.5 (3.9)} \\ 
\textbf{17} & 76.0 (1.2) & \textbf{77.2 (0.9)*} & \textbf{81.6 (1.0)} & 79.8 (1.0) & \textbf{83.5 (0.8)*} & 83.3 (0.6) & \textbf{82.7 (0.7)*} & 82.0 (0.9) & 75.8 (1.9) & \textbf{77.5 (1.4)*} & 83.1 (0.9) & \textbf{83.2 (0.9)} & \textbf{82.5 (1.0)*} & 81.4 (1.2) \\ 
\textbf{18} & \textbf{90.9 (0.9)*} & 90.3 (1.3) & \textbf{92.2 (0.9)} & 91.8 (1.1) & 94.0 (1.0) & \textbf{94.1 (1.2)} & \textbf{92.8 (1.1)} & 92.4 (1.3) & 88.1 (1.8) & \textbf{88.4 (1.8)} & \textbf{93.3 (1.0)} & 92.8 (1.1) & \textbf{94.1 (0.9)} & 93.8 (0.9) \\ 
\textbf{19} & \textbf{78.3 (3.5)*} & 73.4 (5.2) & \textbf{78.8 (3.7)*} & 74.5 (4.9) & \textbf{79.4 (4.2)*} & 75.8 (4.7) & 74.6 (5.3) & \textbf{74.7 (5.0)} & 68.4 (6.8) & \textbf{70.1 (7.8)} & 75.0 (6.3) & \textbf{75.2 (5.5)} & \textbf{78.8 (3.4)*} & 75.6 (5.1) \\ 
\textbf{20} & \textbf{97.4 (2.3)} & 97.2 (2.4) & \textbf{97.4 (2.3)} & 97.3 (2.3) & \textbf{97.7 (2.0)} & 97.3 (2.6) & \textbf{95.0 (4.0)} & 94.1 (3.8) & \textbf{94.0 (4.0)} & 93.8 (3.2) & \textbf{95.0 (4.0)} & 94.1 (3.8) & \textbf{97.7 (2.0)*} & 96.8 (2.3) \\ 
\hline
\textbf{Average} & \multicolumn{1}{c}{\textbf{79.61 (2.5)}} & 79.16 (2.6) & \multicolumn{1}{c}{\textbf{82.07 (2.2)}} & 81.3 (2.6) & \multicolumn{1}{c}{\textbf{79.75 (2.7)}} & 79.69 (2.9) & \multicolumn{1}{c}{79.72 (3)} & \textbf{80.21 (3.1)} & \multicolumn{1}{c}{76.15 (6.6)} & \textbf{77.45 (5.6)}& \multicolumn{1}{c}{78.41 (3.6)} & \textbf{78.81 (3.6)} & \multicolumn{1}{c}{\textbf{81.31 (3.2)}} & 80.98 (3.1)  \\
\textbf{Difference} &  & -0.45 (0.1) & & -0.77 (0.4) &  & -0.06 (0.2) &  & 0.49 (0.1)  &  & \textbf{1.3 (1)} &  & 0.4 (0) &  & -0.33 (0.1)   \\ \hline

\end{tabular}
}

\end{table*}


==> result_table_max_accuracy.tex <==
\begin{table*}[]
\caption{Comparison of the proposed method for pool generation based on diversity in the complexity space,Generation Choice by Global Accuracy. The results of the mean and standard deviation winners are highlighted.The asterisk represents where there was difference in Wilcoxon}
\label{tab:tabresultacc}
\resizebox{\textwidth}{!}{
\scalefont{0.6}
\centering
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{ l c c c c c c c c c c c c c c}

\hline
\textbf{} & \multicolumn{ 2}{c}{\textbf{All}} & \multicolumn{ 2}{c}{\textbf{LCA}} & \multicolumn{ 2}{c}{\textbf{OLA}} & \multicolumn{ 2}{c}{\textbf{Rank}} & \multicolumn{ 2}{c}{\textbf{Knora-E}} & \multicolumn{ 2}{c}{\textbf{Knora-U}} & \multicolumn{ 2}{c}{\textbf{Meta-Des}} \\ 
 \hline
\textbf{Dataset} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} & \textbf{Bagging} & \textbf{Method} \\ 
\hline \\ 

    % 06 & Faults & 1941 &  27  & 7       & UCI     \\
\textbf{1} & 86.9(2.1) & \textbf{87.8(2.2)} & 82.9(2.7) & \textbf{84.6(3.4)} & 82.9(1.9) & \textbf{83.0(2.2)} & \textbf{81.4(2.7)*} & 81.1(2.9) & 82.2(3.1) & \textbf{82.3(3.1)*} & 86.9(2.3) & \textbf{87.5(2.3)} & 86.2(2.5) & \textbf{86.2(2.7)} \\
\textbf{2} & 84.6(1.4) & \textbf{84.7(1.3)} & \textbf{95.7(0.9)} & \textbf{95.7(1.0)} & \textbf{97.4(0.6)} & \textbf{97.4(0.7)} & \textbf{96.9(0.8)} & \textbf{96.9(0.8)*} & \textbf{96.9(0.7)} & \textbf{96.9(0.8)} & \textbf{96.2(1.0)} & \textbf{96.1(1.0)} & 93.3(1.2) & \textbf{94.4(1.1)*} \\
\textbf{3} & \textbf{77.6(2.0)} & 77.1(3.3) & \textbf{70.4(5.3)} & 68.9(3.9) & 74.8(2.5) & \textbf{75.2(3.3)} & 69.8(3.7) & \textbf{70.0(4.2)} & 70.2(3.8) & \textbf{70.3(4.1)} & \textbf{78.7(1.6)} & 78.3(2.4) & \textbf{76.0(0.9) }& \textbf{76.0(1.1)} \\
\textbf{4} & 81.1(24.3) & \textbf{88.9(1.7)} & 86.2(1.9) & \textbf{86.8(1.8)} & 89.0(1.4) & \textbf{89.3(1.2)} & 88.9(1.6) & \textbf{89.3(1.4)*} & 89.5(1.6) & \textbf{89.8(1.5)} & 89.0(2.1) & \textbf{89.5(1.0)} & 88.8(1.1) & \textbf{89.4(1.2)*} \\
\textbf{5} & 76.8(2.8) & \textbf{76.9(3.0)} & \textbf{70.7(3.1)} & 69.9(3.3) & 72.4(2.6) & \textbf{73.3(3.3)} & 71.5(2.6) & \textbf{71.8(2.6)} & 72.5(2.7) & \textbf{73.1(2.4)} & 76.9(2.7) & \textbf{77.0(2.7)} & 73.7(2.5) & \textbf{74.5(3.3)} \\
\textbf{6} & 69.4(1.7) & \textbf{70.7(2.1)} & 62.8(2.4) & \textbf{64.5(1.9)} & \textbf{67.7(1.9)} & 67.4(1.5) & \textbf{67.4(2.1)} & 67.2(1.8) & \textbf{68.9(1.7)*} & 68.6(2.0) & 71.7(1.5) & \textbf{72.3(1.6)} & 70.3(1.4) & \textbf{70.8(1.3)} \\
\textbf{7} & 75.9(2.3) & \textbf{77.0(2.4)} & 69.1(2.2) & \textbf{70.1(2.6)*} & \textbf{71.2(2.3)} & 70.4(2.1) & \textbf{71.0(2.7)} & 69.4(1.9) & \textbf{72.4(2.3)} & 71.0(1.5) & 76.1(2.4) & \textbf{76.9(2.4)*} & 72.9(1.7) & \textbf{73.0(2.0)} \\
\textbf{8} & 75.0(2.3) & \textbf{76.8(3.3)} & \textbf{69.0(7.8)*} & 62.0(7.4) & \textbf{69.7(4.5)} & 69.5(4.4) & 65.7(5.2) & \textbf{66.0(5.1)} & 65.6(6.1) & \textbf{67.2(4.8)*} & 75.1(2.1) & \textbf{76.4(3.3)} & \textbf{74.0(1.5)*} & 73.4(1.6) \\
\textbf{9} & 82.5(3.7) & \textbf{85.9(3.9)*} & 75.7(7.1) & \textbf{80.1(5.5)} & 77.5(4.5) & \textbf{78.5(4.6)} & 77.1(4.5) & \textbf{77.5(4.1)*} & 79.4(4.2) & \textbf{80.9(4.6)*} & 82.8(3.8) & \textbf{85.5(4.2)} & 82.9(4.0) & \textbf{84.6(3.6)*} \\
\textbf{10} & \textbf{71.4(2.7)} & 70.6(3.7) & 66.8(4.8) & \textbf{69.7(2.1)} & 69.0(3.5) & \textbf{69.3(3.0)} & \textbf{68.0(2.8)} & 67.7(3.8) & \textbf{68.9(2.3)} & 67.9(3.0) & \textbf{71.0(2.4)} & 70.9(2.4) & 70.7(1.6) & \textbf{70.7(2.2)} \\
\textbf{11} & 89.2(2.9) & \textbf{89.9(2.7)*} & 85.4(3.9) & \textbf{87.1(2.5)} & 85.9(2.7) & \textbf{88.8(2.8)*} & 86.0(2.8) & \textbf{88.8(2.9)} & 88.4(3.6) & \textbf{88.8(3.7)*} & 89.2(2.8) & \textbf{90.7(3.1)*} & 88.8(3.0) & \textbf{90.3(2.7)*} \\
\textbf{12} & 83.5(3.7) & \textbf{86.0(5.1)*} & 77.6(6.8) & \textbf{82.5(3.6)*} & 80.6(3.7) & \textbf{81.3(3.8)} & 78.6(3.5) & \textbf{81.3(3.9)*} & 79.9(3.7) & \textbf{82.5(3.9)*} & 83.0(3.9) & \textbf{85.6(4.9)*} & 83.0(5.5) & \textbf{84.5(4.4)} \\
\textbf{13} & 72.7(2.3) & \textbf{76.3(3.2)*} & \textbf{68.1(4.4)} & 67.6(4.4) & \textbf{68.0(4.8)} & 67.3(4.2) & 64.1(5.8) & \textbf{64.3(5.2)} & \textbf{66.7(4.0)} & 66.5(4.6) & 73.5(2.1) & \textbf{75.1(3.0)} & 71.1(2.8) & \textbf{71.2(3.0)} \\
\textbf{14} & 82.8(1.7) & \textbf{82.9(1.7)*} & 92.6(1.0) & \textbf{92.8(1.1)} & \textbf{96.7(0.7)} & 96.6(0.8) & \textbf{96(0.9)} & 95.9(0.8)* & \textbf{96.0(0.7) }& \textbf{96.0(0.7)} & \textbf{95.1(1.1)} & 94.8(1.1) & \textbf{94.2(1.1)} & 94.1(1.0) \\
\textbf{15} & 68.7(4.2) & \textbf{70.5(3.3)*} & 55.3(5.3) & \textbf{57.9(5.5)} & \textbf{68.2(3.9)} & 66.6(5.0) & \textbf{66.4(4.1)} & 66.2(4.3) & \textbf{67.0(4.1)} & 65.6(4.9) & 70.1(3.5) & \textbf{72.1(3.8)} & 67.2(4.7) & \textbf{67.7(4.8)} \\
\textbf{16} & 82.9(2.1) & \textbf{84.0(2.3)} & \textbf{79.7(3.6)} & 74.1(5.4) & 80.8(2.6) & \textbf{81.1(2.2)} & \textbf{77.4(2.4)*} & 77.1(2.7) & 77.2(2.7) & \textbf{77.4(2.8)*} & 82.9(1.9) & \textbf{83.3(2.3)} & 79.7(3.0) & \textbf{79.9(3.3)} \\
\textbf{17} & 78.9(3.2) & \textbf{85.7(2.3)*} & \textbf{72.8(4.3)} & \textbf{72.8(2.9)} & 85.7(3.6) & \textbf{87.6(3.2)} & 85.5(3.8) & \textbf{87.8(3.4)} & 88.9(3.1) & \textbf{89.4(3.1)} & 81.8(3.5) & \textbf{87.3(1.9)*} & 91.5(4.5) & \textbf{94.4(3.2)*} \\
\textbf{18} & 75.6(1.1) & \textbf{77.6(1.1)} & 75.7(2.4) & \textbf{76.5(2.4)*} & \textbf{82.8(0.6)*} & 82.4(0.8) & \textbf{83.0(0.8)} & 82.8(0.8) & \textbf{83.5(0.9)} & 83.1(0.8) & \textbf{81.8(1.0)} & 81.7(0.9) & \textbf{82.5(0.9)} & 82.4(1.0) \\
\textbf{19} & \textbf{56.5(4.6)*} & 54.5(3.2) & 73.4(3.0) & \textbf{74.7(2.8)} & \textbf{88.1(1.7)} & 88.0(1.7) & \textbf{90.1(1.7)*} & 89.7(1.5) & \textbf{90.5(1.6)} & 90.0(1.5) & \textbf{87.2(2.8)} & 86.3(2.5) & \textbf{86.8(2.5)} & 86.7(2.6) \\
\textbf{20} & \textbf{91.0(1.2)*} & 90.8(1.0) & \textbf{88.7(1.2)} & 88.5(1.4) & \textbf{92.8(1.4)} & 92.6(1.2) & \textbf{93.0(1.1)} & 92.8(1.3) & \textbf{94.2(1.0)} & 94.0(1.1) & \textbf{92.3(1.0)} & 91.9(1.0) & \textbf{94.0(1.1)} & \textbf{94.0(1.0)} \\
\textbf{21} & 77.7(3.4) & \textbf{84.4(6.2)*} & 66.9(6.8) & \textbf{73.2(6.9)*} & 75.1(6.2) & \textbf{77.7(6.5)} & 74.8(5.5) & \textbf{77.5(7.2)*} & 78.5(3.5) & \textbf{83.2(6.3)*} & 78.1(3.0) & \textbf{84.8(6.3)} & 79.7(3.7) & \textbf{84.9(5.3)*} \\
\textbf{22} & 96.6(1.2) & \textbf{97.1(1.0)} & \textbf{95.0(1.9)} & 94.4(1.4) & 95.7(1.7) & \textbf{96.1(1.3)} & 95.1(1.7) & \textbf{95.6(1.6)} & 95.9(1.8) & \textbf{96.2(1.6)} & 97.0(1.0) & \textbf{97.2(1.0)} & 96.4(0.9) & \textbf{97.0(0.9)*} \\
\textbf{23} & 75.2(2.0) & \textbf{75.5(2.6)} & 67.1(2.5) & \textbf{68.1(2.3)} & 73.1(2.0) & \textbf{74.0(2.0)} & 73.0(2.0) & \textbf{74.5(2.6)*} & \textbf{75.8(2.2)} & 75.5(2.5) & 76.0(2.1) & \textbf{76.5(2.9)*} & 75.9(2.3) & \textbf{76.2(1.9)} \\
\textbf{24} & 87.1(3.4) & \textbf{89.1(3.8)*} & \textbf{81.7(4.6)} & 81.5(4.2) & 83.8(4.3) & \textbf{85.1(4.0)} & 84.3(5.0) & \textbf{84.6(4.0)} & 84.8(4.3) & \textbf{85.2(3.9)} & 86.5(4.0) & \textbf{88.0(4.2)} & 86.7(3.8) & \textbf{88.0(3.0)} \\
\textbf{25} & 97.1(1.1) & \textbf{98.0(0.8)*} & 95.0(1.4) & \textbf{95.5(1.4)} & 96.0(1.3) & \textbf{96.3(1.1)} & 95.9(1.3) & \textbf{96.2(1.1)} & 97.1(0.9) & \textbf{97.4(1.0)} & 97.1(1.2) & \textbf{98.1(0.7)} & 96.9(1.3) & \textbf{97.2(1.2)*} \\
\textbf{26} & 86.5(0.8) & \textbf{86.8(1.0)*} & 79.2(2.1) & \textbf{80.3(1.6)} & 82.4(1.2) & \textbf{83.0(1.1)} & 82.0(0.9) & \textbf{82.4(1.4)} & 83.4(0.8) & \textbf{83.7(1.0)} & 86.4(0.8) & \textbf{86.8(0.9)} & 85.9(0.8) & \textbf{86.1(0.9)} \\
\textbf{27} & 82.5(3.8) & \textbf{85.3(3.6)*} & 75.4(5.0) & \textbf{78.7(4.9)} & 79.7(4.5) & \textbf{81.4(4.1)} & 79.9(4.7) & \textbf{81.3(4.7)} & 82.1(4.6) & \textbf{82.9(3.8)*} & 83.2(3.6) & \textbf{85.2(3.8)} & 82.7(3.4) & \textbf{85.3(3.4)*} \\
\textbf{28} & 97.5(2.3) & \textbf{98.4(1.9)*} & 94.2(4.3) & \textbf{97.0(1.9)*} & 95.0(2.2) & \textbf{97.3(2.0)*} & 95.0(2.2) & \textbf{97.3(2.0)*} & 97.5(2.0) & \textbf{98.4(1.9)*} & 97.5(2.1) & \textbf{98.5(1.8)*} & 98.0(2.0) & \textbf{98.4(1.9)} \\ \hline
\textbf{Aver.} & \multicolumn{1}{r}{80.83} & \textbf{82.47} & \multicolumn{1}{r}{77.61} & \textbf{78.41} & \multicolumn{1}{r}{81.5} & \textbf{82.02} & \multicolumn{1}{r}{80.64} & \textbf{81.18} & \multicolumn{1}{r}{81.93} & \textbf{82.28} & \multicolumn{1}{r}{83.68} & \textbf{84.8} & \multicolumn{1}{r}{83.21} & \textbf{83.98} \\ 
\textbf{Diff.} &  & -1.64 &  & -0.8 &  & -0.52 &  & -0.54 &  & -0.35 &  & -1.12 &  & -0.77 \\ \hline


\hline
\end{tabular}
}

\end{table*}

